A Proposed Set of Communicative Gestures for Human Robot Interaction and an RGB Image-based Gesture Recognizer Implemented in ROS

We propose a set of communicative gestures and develop a gesture recognition system with the aim of facilitating more intuitive Human-Robot Interaction (HRI) through gestures. First, we propose a set of commands commonly used for human-robot interaction. Next, an online user study with 190 participants was performed to investigate if there was an agreed set of gestures that people intuitively use to communicate the given commands to robots when no guidance or training were given. As we found large variations among the gestures exist between participants, we then proposed a set of gestures for the proposed commands to be used as a common foundation for robot interaction. We collected ~7500 video demonstrations of the proposed gestures and trained a gesture recognition model, adapting 3D Convolutional Neural Networks (CNN) as the classifier, with a final accuracy of 84.1% (sigma=2.4). The resulting model was capable of training successfully with a relatively small amount of training data. We integrated the gesture recognition model into the ROS framework and report details for a demonstrated use case, where a person commands a robot to perform a pick and place task using the proposed set. This integrated ROS gesture recognition system is made available for use, and built with the intention to allow for new adaptations depending on robot model and use case scenarios, for novel user applications.

==> Text/archive_figures.tex <==
% \begin{table}[b]
% \label{table:performance}
%     \caption{Model accuracy with different training dataset sizes}
%     \centering
%     \label{table:performance}
%     \begin{tabular}{|c|c|c|c|c|}
%         \hline
%             Number of videos & \multicolumn{2}{ c |}{Stage 1 Dataset}  & \multicolumn{2}{ c |}{Stage 2 Dataset}  \\ 
%             \cline{2-5} per gesture & Accuracy & Recall & Accuracy & Recall   \\ \hline
%             $\sim50$  & $17.1\pm{3.3}\%$    & $19.6\pm{2.2}\%$   & $81.0\pm{1.3}\%$   & $81.9\pm{2.2}\%$                          \\ %\hline
%             $\sim100$ & $19.7\pm{2.6}\%$    & $21.3\pm{3.1}\%$   & $79.2\pm{2.1}\%$   & $80.2\pm{2.5}\%$                          \\ %\hline
%             $\sim150$ & $21.2\pm{2.2}\%$    & $23.4\pm{1.5}\%$   & $82.3\pm{1.9}\%$    & $83.1\pm{1.7}\%$                          \\ %\hline
%         \hline
%     \end{tabular}
% \end{table}

% \begin{table}[b]
% \label{table:continents}
%     \caption{Continents participants was born in and spend most of their time in}
%     \centering
%     \label{table:continents}
%     \begin{tabular}{|c|c|c|}
%         \hline
%             Continent & Continent of Birth & Spend most of their time \\ \hline
%             Africa          & 5.9\%     & 5.9\%     \\ %\hline
%             Asia            & 37.0\%    & 31.9\%    \\ %\hline
%             Europe          & 17.0\%    & 20.7\%    \\ %\hline
%             South America   & 11.9\%    & 12.6\%    \\ %\hline
%             North America   & 17.8\%    & 19.3\%    \\ %\hline
%             Oceania         & 10.4\%    & 9.6\%     \\
%         \hline
%     \end{tabular}
% \end{table}

% \begin{table}[b]
% \label{table:country}
%     \caption{Country participants was born in and spend most of their time in}
%     \centering
%     \begin{tabular}{|c|c|c|}
%         \hline
%             Country & Country of Birth & Spend most of their time \\ \hline
%             Albania             & 0.74\%    & 0\%       \\
%             Andorra             & 0\%       & 0.74\%    \\
%             Australia           & 9.63\%    & 10.37\%   \\
%             Brazil              & 10.37\%   & 10.37\%   \\
%             Burundi             & 0\%       & 0.74\%    \\
%             Canada              & 0.74\%    & 0.74\%    \\
%             China               & 1.48\%    & 0.74\%    \\
%             Cuba                & 0.74\%    & 0\%       \\
%             Czech Republic      & 0.74\%    & 0.74\%    \\
%             France              & 1.48\%    & 1.48\%    \\
%             Germany             & 0.74\%    & 0\%       \\
%             India               & 30.37\%   & 28.89\%   \\
%             Iran                & 0.74\%    & 0.74\%    \\
%             Ireland             & 0\%       & 0.74\%    \\
%             Italy               & 12.59\%   & 16.30\%   \\
%             Kenya               & 2.22\%    & 1.48\%    \\
%             Mexico              & 1.48\%    & 1.48\%    \\
%             Nigeria             & 2.96\%    & 2.96\%    \\
%             Philippines         & 0.74\%    & 0.74\%    \\
%             Russia Federation   & 2.96\%    & 0\%       \\
%             Sri Lanka           & 0.74\%    & 0.74\%    \\
%             Turkey              & 0.74\%    & 0.74\%    \\
%             America             & 17.04\%   & 18.52\%   \\
%             Zimbabwe            & 0.74\%    & 0.74\%    \\
%         \hline
%     \end{tabular}
% \end{table}

% Not sure if you think this is necessary
% \begin{table}[h]
% \label{table:cfn_matrix}
%     \caption{Bottom 5 worst performing gestures}
%     \centering
%     \label{table:cfn_matrix}
%     \begin{tabular}{|c|c|c|}
%         \hline
%             Gesture & Precision & Recall \\ \hline
%             Give an Item & 0.75 & 0.67   \\ %\hline
%             Receive an Item & 0.94 & 0.71   \\ %\hline
%             Speed Up & 0.94 & 0.81   \\ %\hline
%             Follow you & 0.97 & 0.83   \\ %\hline
%             Anti-clockwise  & 0.85 & 0.83   \\ %\hline
%         \hline
%     \end{tabular}
% \end{table}

% \begin{figure}[t]
%     \centering
%     \label{fig:stage1}
%     \includegraphics[width=.4\textwidth]{Images/cfn_stage_1.png}
%     \vspace{-3mm}
%     \caption{Confusion matrix generated using training data from Stage 1 of the collection study - gestures curated from participants}
%     \vspace{-5mm}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \label{fig:stage2}
%     \includegraphics[width=.4\textwidth]{Images/cfn_stage_2.png}
%     \vspace{-3mm}
%     \caption{Confusion matrix generated using training data from Stage 2 of the collection study - demonstrated gestures}
%     \vspace{-5mm}
% \end{figure}


% % Figure of two confusion matrices
% \begin{figure*}
%     \centering
%     \label{fig:confusion_matrix}
%     \begin{minipage}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Images/cfn_stage_1.png}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Images/cfn_stage_2.png}
%     \end{minipage}
%     \vspace{-3mm}
%     \caption{Confusion matrix generated using training data from the user study. With Stage 1 results, participant curated gestures, on the left and Stage 2 results, demonstrated gestures, on the right.}
%     \vspace{-5mm}
% \end{figure*}

%In our demonstration \footnote{Demonstration video: https://youtu.be/X1rc98xzlJw}, we successfully sent commands to instruct a mobile manipulator robot to execute arm and base movements, as well as an object grasping and handover task. Moreover, we were able to send commands to pause, resume, or shutdown the gesture recognition interface when desired. This allows the person to specify to the robot when to pay attention to user gestures. A future user study will further substantiate the utility and evaluation of this system once the COVID-19 pandemic has been resolved to allow studies to recommence. 

% Based on Figure 4, the loop begins with the user performing a gesture to signal the robot. The action was then captured by an external camera and forwarded into the gesture recognition model as a ROS topic. Due to the hardware limitations for the Fetch robot, an external computer will be required to run the inference layer of the model. The model will then publish the predicted result to the state machine, instructing the robot to perform specific actions if the right conditions were met. Upon completion, the robot will once again wait for the user to perform the next gesture before executing the next action. By utilising this system, the model shows many potential applications in the HRI space.

% By taking account of the proposed gestures used in the developed gesture recognition model, different poses and actions were configured for the robot to correspond to each gesture. With that in mind, we are able to categorise each gesture as a different form of command for the overall system. These gestures are grouped as followed:

% \begin{table}[b]
%     \vspace{-3mm}
%     \caption{Proposed list of commands for HRI applications}
%     \centering
%     \label{table:gestures}
%     \begin{tabular}{l l l}
%             1. Start                            & 14. Pause              \\ 
%             2. Stop                             & 15. Watch Out          \\
%             3. Handwave                         & 16. Speed up           \\
%             4. Point to an Object               & 17. Slow down          \\ 
%             5. Point to an Area                 & 18. Thumbs up          \\ 
%             6. Give me an item                  & 19. Thumbs down        \\ 
%             7. Receive an item                  & 20. Agree              \\
%             8. Repeat                           & 21. Disagree           \\
%             9. Undo                             & 22. Come forward       \\ 
%             10. Watch Me                        & 23. Move to the left   \\ 
%             11. I will Follow You               & 24. Move to the right  \\
%             12. Follow Me                       & 25. Move backwards     \\
%             13. Resume                          &                        \\
%     \end{tabular}
% \end{table}

% To enable robots to be integrated in society, there is a need to establish a communication protocol to facilitate effective human robot cooperation~\cite{canal_gesture_2015}. Existing research has investigated interactive channels such as voice, speech, gaze, and gestures to facilitate human robot communication \cite{6926324, doi:10.1089/dst.2012.0010, 10.1145/3319502.3374810}. Despite recent advancements in voice and speech recognition, performance has often been dependent on both hardware and software constraints. Most robots are not equipped with speech sensors and require external microphones with  variable performance~\cite{6926324}. Other challenges include the complexity of accents, dialects, ambiguity in context, grammar irregularities, and homophones~\cite{doi:10.1089/dst.2012.0010}, which can cause difficulty in developing generic model that can be implemented in multiple environments. Gaze can also have its own challenges, such as being context-dependent \cite{10.1145/3319502.3374810}, and reliable gaze detection typically requires specialized devices to be strapped onto the user's head, or the user to be relatively stationary. Instead, gestures can be more easily learned and executed by users, and detected using common robot sensors (i.e., RGB cameras), without the aforementioned challenges. A key fact of human communication is the use of gestures and successful mimicry of observed gestures, with a suitable level of accuracy and understanding \cite{haddadi_analysis_2013}. Hence, this paper focuses on the use of communicative gestures for human robot interaction.
